Towards Multimodal Vision-Language Models Generating Non-Generic Text

Vision-language models can assess visual context in an image and generate descriptive text. While the generated text may be accurate and syntactically correct, it is often overly general. To address this, recent work has used optical character recognition to supplement visual information with text extracted from an image. In this work, we contend that vision-language models can benefit from additional information that can be extracted from an image, but are not used by current models. We modify previous multimodal frameworks to accept relevant information from any number of auxiliary classifiers. In particular, we focus on person names as an additional set of tokens and create a novel image-caption dataset to facilitate captioning with person names. The dataset, Politicians and Athletes in Captions (PAC), consists of captioned images of well-known people in context. By fine-tuning pretrained models with this dataset, we demonstrate a model that can naturally integrate facial recognition tokens into generated text by training on limited data. For the PAC dataset, we provide a discussion on collection and baseline benchmark scores.

==> fig/ablation-table.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{8pt}
\begin{table}
    \centering
    \caption{Special Token Feature Ablations}
    \begin{tabular}{
        l
        S[table-format = -.1]
        S[table-format = -.5]
        S[table-format = 1.3]
        S[table-format = -.2]
        S[table-format = 1.3]
        S[table-format = 1.3]
        S[table-format = 2.2]
        }
        \toprule
        \multicolumn{3}{c}{} & 
        \multicolumn{5}{c}{PAC Test Set Metrics}\\
        \cmidrule(lr){2-6}        
        {Model} &{{B-4}}& {M} & {R} & {S} & {C}\\
        \midrule
        M4C & {-}  & {-}  & {-}  & {-}  & {-}   \\
        M4C with Source Feat & {-}  & {-}  & {-}  & {-}  & {-}   \\
        FastText & {-}  & {-}   & {-}  & {-}  & {-}  \\
        FasterRCNN  &  {-} & {-}  & {-}  & {-}  & {-}  \\
        Bounding Box &  {-} & {-} & {-} & {-} & {-}  \\
        Source Feature &  {-} & {-} & {-} & {-} & {-}  \\
        \bottomrule
    \end{tabular}
\end{table}


==> fig/base-table.tex <==
\setlength{\tabcolsep}{7pt}

\begin{table*}[h]
    
    \centering
    \caption{\label{table:base} PAC Baselines using Special Tokens and M4C Architecture. In the training column, a $\rightarrow$ between datasets indicates one dataset was trained on before the other where as a comma in between datasets indicates they were trained on simultaneously. Datasets trained on simultaneously are followed by a sampling ratio between datasets(e.g PAC,TextCaps[1:8] is 1 batch of PAC per 8 batches of TextCaps).}
    \begin{tabular*}{0.90\textwidth}{@{\extracolsep{\fill}}llllrrrrr}
    
        \toprule
        \multicolumn{3}{c}{} & 
        \multicolumn{6}{c}{Metrics}\\
        \cmidrule(lr){5-9}        
        \# & {Tokens} & {Training} & {{Test}} & {{B-4}} & {M} & {R} & {C} & {S}\\
        \midrule
        % {1 a.} & {OCR Only}       & {TextCaps$\rightarrow$PAC} & {PAC}& 14.5  & 22.4 & 42.0 & 156.8 & 30.3  \\
        % {\hspace{3}\hphantom{1}b.} &  & &                       {TextCaps} & 20.7  & 20.1 & 43.0 & 80.4 & 13.4 \\
        {1 a.} & {Special}       & {TextCaps} & {PAC}& 0.7  & 5.1 & 11.7 & 10.4 & 3.0  \\
        {\hspace{3mm}b.} & & & {TextCaps \hphantom{1mm}}& 22.9  & 22.1 & 46.0 & 89.7 & 15.3 \\    
        {2 a.} & {Special}       & {PAC} & {PAC}& 8.6  & 13.3 & 29.1 & 98.9 & 17.6  \\
        {\hspace{3mm}b.} &  & &                       {TextCaps} & 2.0  & 7.5 & 22.0 & 8.5 & 2.6 \\
        {3 a.} & {Special}       & {TextCaps$\rightarrow$PAC} & {PAC}& 9.1  & 14.8 & 30.4 & 102.6 & 18.7  \\
        {\hspace{3mm}b.} &  & &                       {TextCaps} & 20.7  & 20.1 & 43.0 & 80.4 & 13.4 \\
        {4 a.} & {Special}                     & {PAC,TextCaps[1:8]} & {PAC} & 8.4  & 14.5 & 30.3 & 103.7 & 17.5  \\
        {\hspace{3mm}b.} &  &                       & {TextCaps} & 22.1  & 20.9 & 45.3 & 84.5 & 24.0 \\
        {5 a.} & {Special}  & {TextCaps$\rightarrow$PAC,TextCaps[1:1]} &  {PAC} & 5.1  & 12.8 & 25.7 & 73.0 & 14.8  \\
        {\hspace{3mm}b.} &  &  & {TextCaps} &  23.2 & 22.0 & 46.2 & 91.0 & 15.1 \\
        \bottomrule
        \multicolumn{6}{c}{\footnotesize B-4: BLEU-4; M: METEOR; R: ROUGUE; C: CIDEr, S: SPICE}
    \end{tabular*}
\end{table*}


==> fig/change-table.tex <==
\setlength{\tabcolsep}{14pt}

\begin{table*}[h]
    
    \centering
    \caption{\label{table:change} Training on PAC with and without special tokens. }
    \begin{tabular*}{0.9\textwidth}{@{\extracolsep{\fill}}lllrrrrr}
        \toprule
        \multicolumn{3}{c}{} & 
        \multicolumn{5}{c}{PAC Test Set Metrics}\\
        \cmidrule(lr){4-8}        
        \# & {Model} & {Training} & {B-4} & {M} & {R} & {C} & {S}\\
        \midrule
        {1} & {M4C}   & {TextCaps$\rightarrow$PAC} & 2.1  & 6.4 & 14.3 & 24.6 & 4.3  \\
        % {2} & {M4C+STM} \\
        {2} & {M4C+ST}& {TextCaps$\rightarrow$PAC} & 9.1 & 14.8 & 30.4 & 102.6 & 18.7  \\
        \bottomrule
        \multicolumn{6}{c}{\footnotesize ST: Special Tokens; B-4: BLEU-4; M: METEOR; R: ROUGUE; C: CIDEr, S: SPICE}
    \end{tabular*}
\end{table*}


==> fig/img-fig.tex <==
\begin{figure*}[h]
\centering
\includegraphics[scale=.45]{assets/textcaps-pac.png}
\caption{\label{fig:capspac} In both human captions, non-generic terms are used. Incorporation of external vocabulary tokens is decisive to whether a vision-language model can generate similar text.}
\end{figure*}


==> fig/textcaps-table.tex <==
\renewcommand{\arraystretch}{1.2}

\begin{table}
\setlength{\tabcolsep}{1pt}
    \centering
    \caption{TextCaps Baselines. The model in row #2 is used for subsequent benchmarks.}
    \begin{tabular}{
        l
        S[table-format = -.1]
        S[table-format = -.5]
        S[table-format = 1.3]
        S[table-format = -.2]
        S[table-format = 1.3]
        S[table-format = 1.3]
        S[table-format = 2.2]
        }
        \toprule
        \multicolumn{3}{c}{} & 
        \multicolumn{5}{c}{TextCaps Val Set Metrics}\\
        \cmidrule(lr){3-7}        
        {Num.} & {Model} &{{B-4}}& {M} & {R} & {S} & {C}\\
        \midrule
        1 & {M4C} & 23.2  & 22.1  & 46.2  & 91.7  & 15.4   \\
        2 & {M4C+SF} & {-}  & {-}  & {-}  & {-}  & {-}   \\
        \bottomrule
        \multicolumn{6}{c}{\footnotesize B-4: BLEU-4; M: METEOR; R: ROUGUE; S: SPICE; C: CIDEr} \\
        \multicolumn{2}{c}{\footnotesize SF: source feature}
    \end{tabular}
    \label{table:textcaps}
\end{table}


==> fig/tiane-fig.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{assets/tsne.png}
\caption{\label{fig:teaser} Our model accepts tokens from several upstream classifiers, learns representations for tokens from different classifiers, and uses each token appropriately in image captions. By using the facial recognition token `Bernie Sanders', our model's caption is more informative and meaningful than previous work that just uses OCR.}
\end{figure}

